Explicit Effect Subtyping

As popularity of algebraic effects and handlers increases, so does a demand for their efficient execution. Eff, an ML-like language with native support for handlers, has a subtyping-based effect system on which an effect-aware optimizing compiler could be built. Unfortunately, in our experience, implementing optimizations for Eff is overly error-prone because its core language is implicitly-typed, making code transformations very fragile. To remedy this, we present an explicitly-typed polymorphic core calculus for algebraic effect handlers with a subtyping-based type-and-effect system. It reifies appeals to subtyping in explicit casts with coercions that witness the subtyping proof, quickly exposing typing bugs in program transformations. Our typing-directed elaboration comes with a constraint-based inference algorithm that turns an implicitly-typed Eff-like language into our calculus. Moreover, all coercions and effect information can be erased in a straightforward way, demonstrating that coercions have no computational content. Additionally, we present a monadic translation from our calculus into a pure language without algebraic effects or handlers, using the effect information to introduce monadic constructs only where necessary.

==> Figures/source-type-elaboration.tex <==
%% || \textbf{Value Type Elaboration} $\ruleform{\elabVty{\polyTy} = \vty}$
%% || \textbf{Computation Type Elaboration} $\ruleform{\elabCty{\cCty} = \cty}$
%% || \textbf{Constraint Elaboration} $\ruleform{\elabConstraint{\srcFullCt} = \trgFullCt}$
%% || \textbf{Typing Environment Elaboration} $\ruleform{\elabTyEnv{\tyEnv} = \tyEnv'}$
\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{10mm}}c@{\hspace{0mm}}}
  \begin{array}{@{\hspace{0mm}}lcl@{\hspace{0mm}}}
    % Type Variable
    \elabVty{\tyvar}                            & = & \tyvar \\
    % Arrow Type
    \elabVty{\aVty \to \cCty}                   & = & \elabVty{\aVty} \to \elabCty{\cCty} \\
    % Handler Type
    \elabVty{\cCty \hto \dCty}                  & = & \elabCty{\cCty} \to \elabCty{\dCty} \\
    % Unit Type
    \elabVty{\tyUnit}                           & = & \tyUnit \\
    % Skeleton Abstraction
    \elabVty{\forall \evar. \polyTy}            & = & \forall \evar. \elabVty{\polyTy} \\
    % Type Abstraction
    \elabVty{\forall \tyvar : \ety. \polyTy}    & = & \forall \tyvar : \ety. \elabVty{\polyTy} \\
    % Dirt Abstraction
    \elabVty{\forall \dirtvar. \polyTy}         & = & \forall \dirtvar. \elabVty{\polyTy} \\
    % Constraint Abstraction
    \elabVty{\srcPartialCt \Rightarrow \qualTy} & = & \elabConstraint{\srcPartialCt} \Rightarrow \elabVty{\qualTy} \\
  \end{array}
&
  \begin{array}{@{\hspace{0mm}}lcl@{\hspace{0mm}}}
    \elabCty{\aVty\,!\,\dirt}                   & = & \elabVty{\aVty}\,!\,\dirt \\
    \\
    \elabTyEnv{\epsilon}                        & = & \epsilon \\
    \elabTyEnv{\tyEnv, \evar}                   & = & \elabTyEnv{\tyEnv}, \evar \\
    \elabTyEnv{\tyEnv, \tyvar : \ety}           & = & \elabTyEnv{\tyEnv}, \tyvar : \ety \\
    \elabTyEnv{\tyEnv, \dirtvar}                & = & \elabTyEnv{\tyEnv}, \dirtvar \\
    \elabTyEnv{\tyEnv, x : \polyTy}             & = & \elabTyEnv{\tyEnv}, x : \elabVty{\polyTy} \\
    \elabTyEnv{\tyEnv, \covar : \srcFullCt}     & = & \elabTyEnv{\tyEnv}, \covar : \elabConstraint{\srcFullCt} \\
  \end{array}
\end{array}
\]
\[
\begin{array}{lcl}
  % Value Type Constraint
  \elabConstraint{\aVty \le \bVty} & = & \elabVty{\aVty} \le \elabVty{\bVty} \\
  % Computation Type Constraint
  \elabConstraint{\cCty \le \dCty} & = & \elabCty{\cCty} \le \elabCty{\dCty} \\
  % Dirt Constraint
  \elabConstraint{\dirt_1 \le \dirt_2} & = & \dirt_1 \le \dirt_2 \\
\end{array}
\]


==> Figures/source-well-formedness.tex <==
$\ruleform{\tcElabPolyTy{\tyEnv}{\aVty}{\ety}{\vty}}$ \textbf{Value Type Well-formedness}
\begin{mathpar}
% Type Variable
\inferrule*[right=]%WfTyVar]
           { \tyvar\!:\!\ety \in \tyEnv }
           { \tcElabPolyTy{\tyEnv}{\tyvar}{\ety}{\tyvar} }

% Arrow Type
\inferrule*[right=]%WfTyArr]
           { \tcElabPolyTy{\tyEnv}{\aVty}{\ety_1}{\vty} \\
             \tcElabCompTy{\tyEnv}{\cCty}{\ety_2}{\cty}
           } % Premises end here
           { \tcElabPolyTy{\tyEnv}{\aVty \to \cCty}{\ety_1 \to \ety_2}{\vty \to \cty} }

% Handler Type
\inferrule*[right=]%WfHandTy]
           { \tcElabCompTy{\tyEnv}{\cCty}{\ety_1}{\cty_1} \\
             \tcElabCompTy{\tyEnv}{\dCty}{\ety_2}{\cty_2}
           } % Premises end here
           { \tcElabPolyTy{\tyEnv}{\cCty \hto \dCty}{\ety_1 \hto \ety_2}{\cty_1 \hto \cty_2} }

% Unit Type
\inferrule*[right=]%WfUnitTy]
           { }
           { \tcElabPolyTy{\tyEnv}{\tyUnit}{\tyUnit}{\tyUnit} }

% Constraint Abstraction
\inferrule*[right=]%WfCoAbsTy]
           { \tcElabConstraint{\tyEnv}{\srcPartialCt}{\trgPartialCt} \\
             \tcElabPolyTy{\tyEnv}{\qualTy}{\ety}{\vty}
           } % Premises end here
           { \tcElabPolyTy{\tyEnv}{\srcPartialCt \Rightarrow \qualTy}{\ety}{\trgPartialCt \Rightarrow \vty} }

% Type Abstraction
\inferrule*[right=]%WfTyAbs]
           { \tcElabPolyTy{\tyEnv, \tyvar:\ety_1}{\polyTy}{\ety_2}{\vty} }
           { \tcElabPolyTy{\tyEnv}{\forall \tyvar\!:\!\ety_1. \polyTy}{\ety_2}{\forall \tyvar\!:\!\ety_1. \vty} }

% Dirt Abstraction
\inferrule*[right=]%WfDirtAbs]
           { \tcElabPolyTy{\tyEnv, \dirtvar}{\polyTy}{\ety}{\vty} }
           { \tcElabPolyTy{\tyEnv}{\forall \dirtvar. \polyTy}{\ety}{\forall \dirtvar. \vty} }

% Skeleton Abstraction
\inferrule*[right=]%WfSkelAbs]
           { \tcElabPolyTy{\tyEnv, \evar}{\polyTy}{\ety}{\vty} }
           { \tcElabPolyTy{\tyEnv}{\forall \evar. \polyTy}{\forall \evar.\ety}{\forall \evar. \vty} }
\end{mathpar}
% =============================================================================
$\ruleform{\tcElabCompTy{\tyEnv}{\cCty}{\ety}{\cty}}$ \textbf{Computation Type Well-formedness}
\begin{mathpar}
% Computation Type
\inferrule*[right=]%WfCompTy]
           { \tcElabPolyTy{\tyEnv}{\aVty}{\ety}{\vty} \\
             \wfDirt{\tyEnv}{\dirt}
           } % Premises end here
           { \tcElabCompTy{\tyEnv}{\aVty~!~\dirt}{\ety}{\vty~!~\dirt} }
\end{mathpar}
% =============================================================================
$\ruleform{\tcElabConstraint{\tyEnv}{\srcFullCt}{\trgFullCt}}$ \textbf{Constraint Well-formedness}
\begin{mathpar}
% Value Type Constraint
\inferrule*[right=]%WfVTyCt]
           { \tcElabPolyTy{\tyEnv}{\aVty}{\ety}{\vty_1} \\
             \tcElabPolyTy{\tyEnv}{\bVty}{\ety}{\vty_2}
           } % Premises end here
           { \tcElabConstraint{\tyEnv}{\aVty \le \bVty}{\vty_1 \le \vty_2} }

% Computation Type Constraint
\inferrule*[right=]%WfCTyCt]
           { \tcElabCompTy{\tyEnv}{\cCty}{\ety}{\cty_1} \\
             \tcElabCompTy{\tyEnv}{\dCty}{\ety}{\cty_2}
           } % Premises end here
           { \tcElabConstraint{\tyEnv}{\cCty \le \dCty}{\cty_1 \le \cty_2} }

% Dirt Constraint
\inferrule*[right=]%WfDirtCt]
           { \wfDirt{\tyEnv}{\dirt_1} \\
             \wfDirt{\tyEnv}{\dirt_2}
           } % Premises end here
           { \tcElabConstraint{\tyEnv}{\dirt_1 \le \dirt_2}{\dirt_1 \le \dirt_2} }
\end{mathpar}
% =============================================================================
$\ruleform{\wfDirt{\tyEnv}{\dirt}}$ \textbf{Dirt Well-formedness}
\begin{mathpar}
% Empty Dirt
\inferrule*[right=]%WfEmpty]
           { }
           { \wfDirt{\tyEnv}{\emptyset} }

% Dirt Variable
\inferrule*[right=]%WfDirtVar]
           { \dirtvar \in \tyEnv }
           { \wfDirt{\tyEnv}{\dirtvar} }

% Op
\inferrule*[right=]%WfOpDirt]
           { (\op : \aVty_\op \to \bVty_\op) \in \sig \\
             \wfDirt{\tyEnv}{\dirt}
           } % Premises end here
           { \wfDirt{\tyEnv}{\{ \op \} \cup \dirt} }
\end{mathpar}
% =============================================================================
$\ruleform{\tcSkeleton{\tyEnv}{\ety}}$ \textbf{Skeleton Well-formedness}
\begin{mathpar}
% Skeleton Variable
\inferrule*[right=]
           { \evar \in \tyEnv }
           { \tcSkeleton{\tyEnv}{\evar} }

% Unit Type
\inferrule*[right=]
           { }
           { \tcSkeleton{\tyEnv}{\tyUnit} }

% Arrow Type
\inferrule*[right=]
           { \tcSkeleton{\tyEnv}{\ety_1} \\
             \tcSkeleton{\tyEnv}{\ety_2}
           } % Premises end here
           { \tcSkeleton{\tyEnv}{\ety_1 \to \ety_2} }

% Handler Type
\inferrule*[right=]
           { \tcSkeleton{\tyEnv}{\ety_1} \\
             \tcSkeleton{\tyEnv}{\ety_2}
           } % Premises end here
           { \tcSkeleton{\tyEnv}{\ety_1 \hto \ety_2} }
\end{mathpar}


==> Figures/target-typing.tex <==
\[
\begin{array}{r@{~}c@{~}l}
  \text{typing environment}~\ctx & ::= & \epsilon                             \mid
                                         \tyEnv, \evar                        \mid
                                         \tyEnv, \tyvar : \ety                \mid
                                         \tyEnv, \dirtvar                     \mid
                                         \tyEnv, x : \vty                     \mid
                                         \tyEnv, \covar : \trgPartialCt       \\
\end{array}
\]
% =============================================================================
$\ruleform{\tcTrgVal{\tyEnv}{v}{\vty}}$ \textbf{Values}
\begin{mathpar}
% Term Variable
\inferrule*[right=]%TmVar]
           { (x : \vty) \in \tyEnv }
           { \tcTrgVal{\tyEnv}{x}{\vty} }

% Unit
\inferrule*[right=]%TmUnit]
           { }
           { \tcTrgVal{\tyEnv}{\tmUnit}{\tyUnit} }

% Lambda Abstraction
\inferrule*[right=]%TmTmAbs]
           { \tcTrgComp{\tyEnv, x : \vty}{c}{\cty} \\
             \tcTrgVty{\tyEnv}{\vty}{\ety}
           } % Premises end here
           { \tcTrgVal{\tyEnv}{(\fun{x:\vty}{c})}{\vty \to \cty} }

% Cast a Value
\inferrule*[right=]%TmCastV]
           { \tcTrgVal{\tyEnv}{v}{\vty_1} \\
             \tcTrgCo{\tyEnv}{\coercion}{\vty_1 \le \vty_2}
           } % Premises end here
           { \tcTrgVal{\tyEnv}{\cast{v}{\coercion}}{\vty_2} }

% Skeleton Abstraction
\inferrule*[right=]
           { \tcTrgVal{\tyEnv, \evar}{v}{\vty} }
           { \tcTrgVal{\tyEnv}{\Lambda \evar. v}{\forall \evar.\vty} }

% Type Abstraction
\inferrule*[right=]%TmTyAbs]
           { \tcTrgVal{\tyEnv, \tyvar : \ety}{v}{\vty} }
           { \tcTrgVal{\tyEnv}{\Lambda \tyvar : \ety. v}{\forall \tyvar : \ety.\vty} }

% Dirt Abstraction
\inferrule*[right=]%TmDirtAbs]
           { \tcTrgVal{\tyEnv, \dirtvar}{v}{\vty} }
           { \tcTrgVal{\tyEnv}{\Lambda \dirtvar. v}{\forall \dirtvar. \vty} }

% Coercion Abstraction
\inferrule*[right=]%TmCoAbs]
           { \tcTrgVal{\tyEnv, \covar : \trgPartialCt}{v}{\vty} \\
             \wfTrgCt{\tyEnv}{\trgPartialCt}
           } % Premises end here
           { \tcTrgVal{\tyEnv}{\Lambda (\covar : \trgPartialCt). v}{\trgPartialCt \Rightarrow \vty} }

% Coercion Application
\inferrule*[right=]%TmCoApp]
           { \tcTrgVal{\tyEnv}{v}{\trgPartialCt \Rightarrow \vty} \\
             \tcTrgCo{\tyEnv}{\coercion}{\trgPartialCt}
           } % Premises end here
           { \tcTrgVal{\tyEnv}{v~\coercion}{\vty} }

% Handler
\inferrule*[right=]%TmHandler]
           { \tcTrgComp{\tyEnv, x : \vty_x}{c_r}{\vty\,!\,\dirt} \\
             \left[
               (\op : \vty_1 \to \vty_2) \in \sig \qquad
               \tcTrgComp{\tyEnv, x : \vty_1, k : \vty_2 \to \vty\,!\,\dirt}{c_\op}{\vty\,!\,\dirt}
             \right]_{\op \in \ops}
           } % Premises end here
           { \tcTrgVal{\tyEnv}{\trgShorthand}{\vty_x~!~\dirt \cup \ops \hto \vty~!~\dirt} }

% Skeleton Application
\inferrule*[right=]
           { \tcTrgVal{\tyEnv}{v}{\forall \evar. \vty} \\\\
             \tcSkeleton{\tyEnv}{\ety}
           } %
           { \tcTrgVal{\tyEnv}{v~\ety}{\vty[\ety/\evar]} }

% Type Application
\inferrule*[right=]%TmTyApp]
           { \tcTrgVal{\tyEnv}{v}{\forall \tyvar : \ety. \vty_1} \\\\
             \tcTrgVty{\tyEnv}{\vty_2}{\ety}
           } %
           { \tcTrgVal{\tyEnv}{v~\vty_2}{\vty_1[\vty_2/\tyvar]} }

% Dirt Application
\inferrule*[right=]%TmDirtApp]
           { \tcTrgVal{\tyEnv}{v}{\forall \dirtvar. \vty} \\\\
             \wfDirt{\tyEnv}{\dirt}
           } % Premises end here
           { \tcTrgVal{\tyEnv}{v~\dirt}{\vty[\dirt/\dirtvar]} }
\end{mathpar}
% =============================================================================
$\ruleform{\tcTrgComp{\tyEnv}{c}{\cty}}$ \textbf{Computations}
\begin{mathpar}
% Term Application
\inferrule*[right=]%TmTmApp]
           { \tcTrgVal{\tyEnv}{v_1}{\vty \to \cty} \\
             \tcTrgVal{\tyEnv}{v_2}{\vty}
           } % Premises end here
           { \tcTrgComp{\tyEnv}{v_1~v_2}{\cty} }

% Let Binding
\inferrule*[right=]%TmLet]
           { \tcTrgVal{\tyEnv}{v}{\vty} \\
             \tcTrgComp{\tyEnv, x : \vty}{c}{\cty}
           } % Premises end here
           { \tcTrgComp{\tyEnv}{\letval{x}{v}{c}}{\cty} }

% Return
\inferrule*[right=]%TmReturn]
           { \tcTrgComp{\tyEnv}{v}{\vty} }
           { \tcTrgComp{\tyEnv}{\return{v}}{\vty~!~\emptyset} }

% Do
\inferrule*[right=]%TmDo]
           { \tcTrgComp{\tyEnv}{c_1}{\vty_1~!~\dirt} \\
             \tcTrgComp{\tyEnv, x : \vty_1}{c_2}{\vty_2~!~\dirt}
           } % Premises end here
           { \tcTrgComp{\tyEnv}{\doin{x}{c_1}{c_2}}{\vty_2~!~\dirt} }

% Operation
\inferrule*[right=]%TmOp]
           { (\op : \vty_1 \to \vty_2) \in \sig \\
             \tcTrgVal{\tyEnv}{v}{\vty_1} \\
             \tcTrgComp{\tyEnv, y : \vty_2}{c}{\vty~!~\dirt} \\
             \op \in \dirt
           } % Premises end here
           { \tcTrgComp{\tyEnv}{\operation{v}{y : \vty_2}{c}}{\vty~!~\dirt} }

% Handle
\inferrule*[right=]%TmHandle]
           { \tcTrgVal{\tyEnv}{v}{\cty_1 \hto \cty_2} \\
             \tcTrgComp{\tyEnv}{c}{\cty_1}
           } % Premises end here
           { \tcTrgComp{\tyEnv}{\withhandle{v}{c}}{\cty_2} }

% Cast a Computation
\inferrule*[right=]%TmCastC]
           { \tcTrgComp{\tyEnv}{c}{\cty_1} \\
             \tcTrgCo{\tyEnv}{\coercion}{\cty_1 \le \cty_2}
           } % Premises end here
           { \tcTrgComp{\tyEnv}{\cast{c}{\coercion}}{\cty_2} }
\end{mathpar}


==> Figures/target-well-formedness.tex <==
$\ruleform{\tcTrgVty{\tyEnv}{\vty}{\ety}}$ \textbf{Value Types}
\begin{mathpar}
% Type Variable
\inferrule*[right=]%WfVTyVar]
           { (\tyvar : \ety)\in \tyEnv }
           { \tcTrgVty{\tyEnv}{\tyvar}{\ety} }

% Arrow Type
\inferrule*[right=]%WfVTyArr]
           { \tcTrgVty{\tyEnv}{\vty}{\ety_1} \\
             \tcTrgCty{\tyEnv}{\cty}{\ety_2}
           } % Premises end here
           { \tcTrgVty{\tyEnv}{\vty \to \cty}{\ety_1 \to \ety_2} }

% Handler Type
\inferrule*[right=]%WfVTyHandler]
           { \tcTrgCty{\tyEnv}{\cty_1}{\ety_1} \\
             \tcTrgCty{\tyEnv}{\cty_2}{\ety_2}
           } % Premises end here
           { \tcTrgVty{\tyEnv}{\cty_1 \hto \cty_2}{\ety_1 \hto \ety_2} }

% Unit Type
\inferrule*[right=]%WfVTyUnit]
           { }
           { \tcTrgVty{\tyEnv}{\tyUnit}{\tyUnit} }

% Constraint Abstraction
\inferrule*[right=]%WfVTyCoAbs]
           { \wfTrgCt{\tyEnv}{\trgPartialCt} \\
             \tcTrgVty{\tyEnv}{\vty}{\ety}
           } % Premises end here
           { \tcTrgVty{\tyEnv}{\trgPartialCt \Rightarrow \vty}{\ety} }

% Skeleton Abstraction
\inferrule*[right=]
           { \tcTrgVty{\tyEnv, \evar}{\vty}{\ety} }
           { \tcTrgVty{\tyEnv}{\forall \evar. \vty}{\forall \evar. \ety} }

% Type Abstraction
\inferrule*[right=]%WfVTyTyAbs]
           { \tcTrgVty{\tyEnv, \tyvar : \ety_1}{\vty}{\ety_2} }
           { \tcTrgVty{\tyEnv}{\forall \tyvar : \ety_1. \vty}{\ety_2} }

% Dirt Abstraction
\inferrule*[right=]%WfVTyDirtAbs]
           { \tcTrgVty{\tyEnv, \dirtvar}{\vty}{\ety} }
           { \tcTrgVty{\tyEnv}{\forall \dirtvar. \vty}{\ety} }
\end{mathpar}
% =============================================================================
$\ruleform{\tcTrgCty{\tyEnv}{\cty}{\ety}}$ \textbf{Computation Types}
\begin{mathpar}
% Computation Type
\inferrule*[right=]%WfCTy]
           { \tcTrgVty{\tyEnv}{\vty}{\ety} \\
             \wfDirt{\tyEnv}{\dirt}
           } % Premises end here
           { \tcTrgCty{\tyEnv}{\vty~!~\dirt}{\ety} }
\end{mathpar}
% =============================================================================
$\ruleform{\wfTrgCt{\tyEnv}{\trgFullCt}}$ \textbf{Coercion Types}
\begin{mathpar}
% Value Type Constraint
\inferrule*[right=]%WfVTyCt]
           { \tcTrgVty{\tyEnv}{\vty_1}{\ety} \\
             \tcTrgVty{\tyEnv}{\vty_2}{\ety}
           } % Premises end here
           { \wfTrgCt{\tyEnv}{\vty_1 \le \vty_2} }

% Computation Type Constraint
\inferrule*[right=]%WfCTyCt]
           { \tcTrgCty{\tyEnv}{\cty_1}{\ety} \\
             \tcTrgCty{\tyEnv}{\cty_2}{\ety}
           } % Premises end here
           { \wfTrgCt{\tyEnv}{\cty_1 \le \cty_2} }

% Dirt Constraint
\inferrule*[right=]%WfDTyCt]
           { \wfDirt{\tyEnv}{\dirt_1} \\
             \wfDirt{\tyEnv}{\dirt_2}
           } % Premises end here
           { \wfTrgCt{\tyEnv}{\dirt_1 \le \dirt_2} }
\end{mathpar}
% =============================================================================
$\ruleform{\wfDirt{\tyEnv}{\dirt}}$ \textbf{Dirts}
\begin{mathpar}
% Empty Set
\inferrule*[right=]%WfDirtEmpty]
           { }
           { \wfDirt{\tyEnv}{\emptyset} }

% Dirt Variable
\inferrule*[right=]%WfDirtVar]
           { \dirtvar \in \tyEnv }
           { \wfDirt{\tyEnv}{\dirtvar} }

% Union
\inferrule*[right=]%WfDirtOp]
           { (\op : \vty_1 \to \vty_2) \in \sig \\
             \wfDirt{\tyEnv}{\dirt}
           } % Premises end here
           { \wfDirt{\tyEnv}{\{ \op \} \cup \dirt} }
\end{mathpar}
% =============================================================================
$\ruleform{\tcSkeleton{\tyEnv}{\ety}}$ \textbf{Skeletons}
\begin{mathpar}
% Skeleton Variable
\inferrule*[right=]
           { \evar \in \tyEnv }
           { \tcSkeleton{\tyEnv}{\evar} }

% Unit Type
\inferrule*[right=]
           { }
           { \tcSkeleton{\tyEnv}{\tyUnit} }

% Arrow Type
\inferrule*[right=]
           { \tcSkeleton{\tyEnv}{\ety_1} \\
             \tcSkeleton{\tyEnv}{\ety_2}
           } % Premises end here
           { \tcSkeleton{\tyEnv}{\ety_1 \to \ety_2} }

% Handler Type
\inferrule*[right=]
           { \tcSkeleton{\tyEnv}{\ety_1} \\
             \tcSkeleton{\tyEnv}{\ety_2}
           } % Premises end here
           { \tcSkeleton{\tyEnv}{\ety_1 \hto \ety_2} }

% Type Abstraction
\inferrule*[right=]
           { \tcSkeleton{\tyEnv, \evar}{\ety} }
           { \tcSkeleton{\tyEnv}{\forall \evar. \ety} }
\end{mathpar}

